SocialDial: A Benchmark for Socially-Aware Dialogue Systems

Dialogue systems have been widely applied in many scenarios and are now more powerful and ubiquitous than ever before. With large neural models and massive available data, current dialogue systems have access to more knowledge than any people in their life. However, current dialogue systems still do not perform at a human level. One major gap between conversational agents and humans lies in their abilities to be aware of social norms. The development of socially-aware dialogue systems is impeded due to the lack of resources. In this paper, we present the first socially-aware dialogue corpus - SocialDial, based on Chinese social culture. SocialDial consists of two parts: 1,563 multi-turn dialogues between two human speakers with fine-grained labels, and 4,870 synthetic conversations generated by ChatGPT. The human corpus covers five categories of social norms, which have 14 sub-categories in total. Specifically, it contains social factor annotations including social relation, context, social distance, and social norms. However, collecting sufficient socially-aware dialogues is costly. Thus, we harness the power of ChatGPT and devise an ontology-based synthetic data generation framework. This framework is able to generate synthetic data at scale. To ensure the quality of synthetic dialogues, we design several mechanisms for quality control during data collection. Finally, we evaluate our dataset using several pre-trained models, such as BERT and RoBERTa. Comprehensive empirical results based on state-of-the-art neural models demonstrate that modeling of social norms for dialogue systems is a promising research direction. To the best of our knowledge, SocialDial is the first socially-aware dialogue dataset that covers multiple social factors and has fine-grained labels.

==> old_introduction.tex <==
\section{Introduction}
% Problems:
% There are no prior dialogue corpora annotated with social relation, social distance, power distance etc.
% High cost when querying GPT3 (NormSage)
% It is unknown how social factors support certain NLP applications, e.g. social norm recogntion and emotion recogntion.


% Key contributions:
% First dialogue corpus in Chinese annotated with social factors for studying social norms.
% A test set with multi-turn human written dialogues annotated with social norms and rich social factors.  (Moral Integrity corpus is two turns and focuses on morality)
% The first synthetic training data generated by ChatGPT.
% Why do we need synthetic training data?
%     * low financial cost because no need to call APIs during testing.
%     * Facilitate research that uses synthetic data for model training.
%     * Preserve privacy.
%     * potential higher performance than using large foundation model alone.
% Investigate differences between synthetic data and human written dialogues.
% Semi-structured norm rules with rich associated social factors, more theoretically grounded from the social science perspective.



Dialogue is a common way to exchange ideas, thoughts, and opinions between two or more people in real-world scenarios.
%%~\cite{bohm1991dialogue}.  
Sustained efforts from both academia and industry have enabled the application of intelligent dialogue systems to many situations. 
In recent years, with the support of neural models and massively available data, current dialogue systems have become more powerful and ubiquitous than ever before. Modern dialogue systems have achieved much empirical success in a number of practical scenarios, including task-oriented dialogues~\cite{zhang2020recent} and open-domain dialogues~\cite{kann-etal-2022-open,INR-083}.

%\noteIZ{What is the difference between chit-chat and open domain?}

\begin{figure}
    \centering  
    \includegraphics[width=0.48\textwidth]{images/sigir2023-intro-2.png}
    \caption{A demonstration of socially-aware dialogue in \ourcorpus. Each dialogue starts with social knowledge profile (in the grey box). Within the dialogue, each turn is annotated with an emotional label and whether it is in violation of specific social norms.}
    \label{fig:intro}
\end{figure}

% \lizhen{Haolan, the example is a bit offensive, could you select another example that shows the norm violation is caused by a lack of knowledge about the target culture. The communicative goal is still cooperative and positive. We need to distinguish ourselves from the \moralInt corpus.}

Current dialogue systems mostly focus on analyzing the textual contents in the dialogues, such as extracting illocutionary goals 
or key-value pairs from utterances, and generating responses based on the conversation history (\ie\ previous utterances). 
They largely ignore the fact that dialogue participants have different social/cultural backgrounds and statuses, and try to achieve perlocutionary goals, such as building relationships, resolving conflicts, and achieving a common understanding. 
We posit that incorporating this social and cultural information into automatic dialogue systems will lead to a better understanding of users' utterances and higher-quality responses. 

%For instance, consider the dialogue in Figure~\ref{fig:intro}.
%\trackIZ{Add something about the example}

% , they ignore \trackIZ{social}\noteIZ{Social, cultural or both?} aspects relevant to the dialogues.
% \noteIZ{The first and the last are common goals that are not social} 


There have been some recent preliminary efforts in investigating social factors in the dialogues. 
For example,~\citep{zhang-etal-2018-personalizing} propose to integrate speaker personas, expressed 
with several sentences (\eg\ ``I am a vegetarian''), into the chit-chat dialogue agents. ~\cite{chawla2021towards,DBLP:conf/acl/LiuZDSLYJH20,chawla2022opponent} focus on extracting the emotion trajectories and objectives from various types of dialogues.~\cite{fung2022normsage} extract social norm rules from large-scale dialogue corpus using large-scale pre-trained language models. However, each of these research efforts only utilizes a particular subset of social factors in the dialogues. Naturally, there 
is a lack of dialogue benchmarks annotated with systematic and comprehensive social factors.

To tackle this research gap, in this paper, we propose a novel socially-aware 
dialogue benchmark \ourcorpus, which consists of a hierarchical social knowledge ontology and a set of high-quality semi-automatically constructed dialogues. Specifically, motivated 
by~\cite{hovy-yang-2021-importance}, we construct the ontology about dialogue participants and their social relationships, dialogue environments, social norms and culture, and dialogue goals. 
Furthermore, we construct dialogues grounded in social knowledge from this ontology. To effectively collect relevant social-aware dialogues, we construct appropriate prompts from the ontology and leverage the recently proposed ChatGPT model to produce sufficiently large synthetic dialogues. We further use the extremely large-scale pre-trained language model GPT3~\cite{NEURIPS2020_1457c0d6} to check the quality of these synthetic dialogues by asking 
``Yes/No'' questions to the GPT3 model. We construct the testing dialogues via crowd-sourcing. We directly ask our human annotators to write multi-turn dialogues that could reflect the social knowledge in the ontology.

We conduct dialogue- and utterance-level social factor detection on our proposed \ourcorpus benchmark using several state-of-the-art pre-trained models, including BERT, RoBERTa, ERNIE, and the popular extremely large GPT3 model. We further focus on the difference between synthetic and human-written dialogues. Finally, we demonstrate the utilities of \ourcorpus benchmark in the emotion classification and social norm recognition tasks.

% by combining human annotation with
% .  construct a 


% with the target  to be considered in our dialogue. 


% The social factors include 
% \emph{speaker} (social status, job, age of each speaker in the dialogue); 
% \emph{social relation between speakers} (\eg\ co-workers, family members); 
% \emph{dialogue context} (situational -- \eg\ work or home, formal or informal, social norms, culture and dialogue goal). 



% Given this ontology, we \trackIZ{randomly select}\noteIZ{Why not all? Why mention this now? too much detail} 
% elements from the ontology to form the prompts for GPT3.

% method: feasibility in ontology, GPT3, BERT checking, prompt generation

% \trackIZ{Problems: overall, the use of terminology is a bit sloppy.
% (1)~pre-deep learning systems considered user models, beliefs, background knowledge in dialogues; 
% (2)~there is confusion between social and cultural;
% (3)~half the goals mentioned are not social -- they are normal communicative goals (illocutionary acts) as opposed to perlocutionary acts focusing on social effects. Example: I order you to sit down -- the illocutionary act is a command, and the perlocutionary act is to make you feel small;
% (4)~goals and preferences are not the same;
% (5)~what social factor is covered by \cite{zhang-etal-2018-personalizing}?
% }




==> tables/prompts.tex <==
\begin{table*}[!t]
\caption{Comparison between \ourcorpus and Other Relevant Dialogue Corpora.}
\begin{adjustbox}{ width=\textwidth,center}
\centering
\begin{tabular}{cccccccc}
\hline
\textbf{Role} & \textbf{Name} & \textbf{Social Distance}   & \textbf{Social Relation} &  \textbf{Location} & \textbf{Formality} & \textbf{Topic} & \textbf{Prompts}\\
\hline
 & multi-turn &   299 & 35.8  & English & persuasion\\
\PersuasionforGood~\cite{wang2019persuasion} & multi-turn & 1017 & 10.43  & English & request, persuasion \\

\bottomrule
\end{tabular}
\end{adjustbox}
\label{tab:prompts}
\end{table*}

